Camera Agnostic Two-Head Network for Ego-Lane Inference

Vision-based ego-lane inference using High-Definition (HD) maps is essential in autonomous driving and advanced driver assistance systems. The traditional approach necessitates well-calibrated cameras, which confines variation of camera configuration, as the algorithm relies on intrinsic and extrinsic calibration. In this paper, we propose a learning-based ego-lane inference by directly estimating the ego-lane index from a single image. To enhance robust performance, our model incorporates the two-head structure inferring ego-lane in two perspectives simultaneously. Furthermore, we utilize an attention mechanism guided by vanishing point-and-line to adapt to changes in viewpoint without requiring accurate calibration. The high adaptability of our model was validated in diverse environments, devices, and camera mounting points and orientations.

==> algorithm.tex <==
\begin{algorithm}[t]
	% \scriptsize
	\algrenewcommand\alglinenumber[1]{\small #1:}
	\caption{Lane-level localization on the \ac{HD} map}
	\label{alg:laneloc}
	\hspace*{\algorithmicindent} \textbf{Input:} ($I_t, \mathbf{X}_t) \in$ \{(Image, \ac{GNSS} pose)\}, t = time \\
	\hspace*{\algorithmicindent} \ac{GNSS} error bound = $r$\\
        \hspace*{\algorithmicindent} \ac{HD} map = $\mathbf{M}$\\
        \hspace*{\algorithmicindent} \ac{DNN} Model = $\mathbf{T}$\\
        \hspace*{\algorithmicindent} Model output: lane number = $c\in\{0,1,2\}$\\
        \hspace*{\algorithmicindent} Model output: uncertainty = $u$, $0\le u \le 1$\\
	\hspace*{\algorithmicindent} Uncertainty thresholds: $\epsilon$\\
        \hspace*{\algorithmicindent} The lane number of lane $l= n(l)$\\
	\hspace*{\algorithmicindent} \textbf{Output:} Refined pose of ego vehicle $\tilde{\mathbf{X}_t}$
	\begin{algorithmic}[1]
            \State $S_t = \{(l,d)|d= \text{distance}(\mathbf{X}_t,l) <r \text{, } l\in\{\text{lane in } \mathbf{M}\}\}$
            \If{$S_t \text{ is } \phi$}
                \State $S_t = S_{t-1}$
            \EndIf
            \State $c_t, u_t = \mathbf{T}(I_t)$
            \If{$u_t > \epsilon$}
                \State $c_t = c_{t-1}$
            \EndIf
            \State L,D = $\argmin\limits_{(l,d)\in S | n(l)\text{ is }c_t} d$
            \If{$L$ is None}
                \State L,D = $\argmin\limits_{(l,d)\in S} d$
            \EndIf
            \State $\tilde{\mathbf{X}}_t = \mathrm{proj}_\mathbf{L}(\mathbf{X_t})$
            \State return $\tilde{\mathbf{X}}_t$
	\end{algorithmic}
\end{algorithm}
